HPS Accelerated Spectral Solvers for Time Dependent Problems

A high-order convergent numerical method for solving linear and non-linear parabolic PDEs is presented. The time-stepping is done via an explicit, singly diagonally implicit Runge-Kutta (ESDIRK) method of order 4 or 5, and for the implicit solve, we use the recently developed "Hierarchial Poincare-Steklov (HPS)" method. The HPS method combines a multidomain spectral collocation discretization technique (a "patching method") with a nested-dissection type direct solver. In the context under consideration, the elliptic solve required in each time-step involves the same coefficient matrix, which makes the use of a direct solver particularly effective. The manuscript describes the methodology and presents numerical experiments.

==> macros.tex <==
\newcommand{\pvct}[1]{\bm{#1}}
\newcommand{\vct}[1]{\bm{\mathsf{#1}}}
\newcommand{\pcc}{\pvct{c}}
\newcommand{\pxx}{\pvct{x}}
\newcommand{\pyy}{\pvct{y}}
\newcommand{\pzz}{\pvct{z}}
\newcommand{\uu}{\vct{u}}
\newcommand{\vv}{\vct{v}}
\newcommand{\ww}{\vct{w}}
\newcommand{\tqq}{\tilde{\vct{q}}}
\newcommand{\ff}{\vct{f}}
\newcommand{\tff}{\tilde{\vct{f}}}
\renewcommand{\AA}{\mtx{A}}
\newcommand{\tAA}{\tilde{\mtx{A}}}
\newcommand{\BB}{\mtx{B}}
\newcommand{\CC}{\mtx{C}}
\newcommand{\DD}{\mtx{D}}
\newcommand{\hatDD}{\hat{\mtx{D}}}
\renewcommand{\SS}{\mtx{S}}
\newcommand{\LL}{\mtx{L}}
\newcommand{\TT}{\mtx{T}}
\newcommand{\UU}{\mtx{U}}
\newcommand{\VV}{\mtx{V}}
\newcommand{\WW}{\mtx{W}}
\newcommand{\XX}{\mtx{X}}

%\newcommand{\mtx}[1]{\mathsf{#1}}
\newcommand{\mtx}[1]{\bm{\mathsf{#1}}}
\newcommand{\bfm}[1]{\mbox{\boldmath ${#1}$}}
\newcommand{\adj}{*}
\newcommand{\mtwo}[4]{\left[\begin{array}{cc} #1 & #2 \\ #3 & #4 \end{array}\right]}
\newcommand{\vtwo}[2]{\left[\begin{array}{cc} #1 \\ #2 \end{array}\right]}
\newcommand{\compi}{{\rm i}}

\newtheorem{thm}{Theorem}[section]
\newtheorem{lemma}[thm]{Lemma}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{corollary}[thm]{Corollary}
\newtheorem{remark}{Remark}
%\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{question}{\sf\textbf{Question}}
\newtheorem{example}{Example}
%\numberwithin{equation}{chapter}
%\numberwithin{section}{chapter}
%\numberwithin{remark}{chapter}
%\numberwithin{figure}{chapter}

%\newcommand{\pgnotate}[1]{{\color{blue}[#1]}}
\newcommand{\pgnotate}[1]{}
\newcommand{\term}[1]{\textit{#1}}
\newcommand{\bigO}{\mathrm{O}}
\newcommand{\emphr}[1]{\textit{\color{red}#1}}
\newcommand{\bfb}[1]{\textbf{\color{blue}#1}}

\newcommand{\pgrule}{\mbox{}\\ \rule{\textwidth}{0.5pt} \\}
\newcommand{\lsp}{\vspace{3mm}}

\newcommand{\mA}{\mtx{A}}
\newcommand{\mB}{\mtx{B}}
\newcommand{\mC}{\mtx{C}}
\newcommand{\mD}{\mtx{D}}
\newcommand{\mE}{\mtx{E}}
\newcommand{\mF}{\mtx{F}}
\newcommand{\mG}{\mtx{G}}
\newcommand{\mH}{\mtx{H}}
\newcommand{\mX}{\mtx{X}}
\newcommand{\mY}{\mtx{Y}}
\newcommand{\mZ}{\mtx{Z}}
\newcommand{\mhA}{\hat{\mtx{A}}}
\newcommand{\mhB}{\hat{\mtx{B}}}
\newcommand{\mhC}{\hat{\mtx{C}}}
\newcommand{\mhD}{\hat{\mtx{D}}}
\newcommand{\mhE}{\hat{\mtx{E}}}
\newcommand{\mhF}{\hat{\mtx{F}}}
\newcommand{\mhG}{\hat{\mtx{G}}}
\newcommand{\mhH}{\hat{\mtx{H}}}
\newcommand{\mhX}{\hat{\mtx{X}}}
\newcommand{\mhY}{\hat{\mtx{Y}}}
\newcommand{\mhZ}{\hat{\mtx{Z}}}
\newcommand{\mtA}{\tilde{\mtx{A}}}
\newcommand{\mtB}{\tilde{\mtx{B}}}
\newcommand{\mtC}{\tilde{\mtx{C}}}
\newcommand{\mtD}{\tilde{\mtx{D}}}
\newcommand{\mtE}{\tilde{\mtx{E}}}
\newcommand{\mtF}{\tilde{\mtx{F}}}
\newcommand{\mtG}{\tilde{\mtx{G}}}
\newcommand{\mtH}{\tilde{\mtx{H}}}
\newcommand{\mtX}{\tilde{\mtx{X}}}
\newcommand{\mtY}{\tilde{\mtx{Y}}}
\newcommand{\mtZ}{\tilde{\mtx{Z}}}
\newcommand{\muA}{\underline{\mtx{A}}}
\newcommand{\muB}{\underline{\mtx{B}}}
\newcommand{\muC}{\underline{\mtx{C}}}
\newcommand{\muD}{\underline{\mtx{D}}}
\newcommand{\muE}{\underline{\mtx{E}}}
\newcommand{\muF}{\underline{\mtx{F}}}
\newcommand{\muG}{\underline{\mtx{G}}}
\newcommand{\muH}{\underline{\mtx{H}}}
\newcommand{\muX}{\underline{\mtx{X}}}
\newcommand{\muY}{\underline{\mtx{Y}}}
\newcommand{\muZ}{\underline{\mtx{Z}}}
\newcommand{\mutB}{\underline{\tilde{\mtx{B}}}}

